Multi-scale Attributed Node Embedding

We present network embedding algorithms that capture information about a node from the local distribution over node attributes around it, as observed over random walks following an approach similar to Skip-gram. Observations from neighborhoods of different sizes are either pooled (AE) or encoded distinctly in a multi-scale approach (MUSAE). Capturing attribute-neighborhood relationships over multiple scales is useful for a diverse range of applications, including latent feature identification across disconnected networks with similar attributes. We prove theoretically that matrices of node-feature pointwise mutual information are implicitly factorized by the embeddings. Experiments show that our algorithms are robust, computationally efficient and outperform comparable models on social networks and web graphs.

==> tables/link_pred.tex <==
\begin{table}[h!]

    \centering
    \footnotesize
    \caption{Link prediction: AUC mean and standard error (100 runs) for best performing (op)erator (best results in bold).}
    \label{tab:link_prediction_1}
    \vspace{2mm}
    \resizebox{.5\textwidth}{!}{
    % \begin{tabular}{lccccccc}
    \begin{tabular}{lccccc}
        \textbf{}    & \textbf{Op.}     &    \textbf{Facebook} & \textbf{GitHub} 
        % & \specialcell{\textbf{Twitch}\\ \textbf{ES}}
        & \specialcell{\textbf{Twitch}\\ \textbf{DE}}
        % & \specialcell{\textbf{Wiki}\\\textbf{Chameleons}}
        & \specialcell{\textbf{Wiki}\\\textbf{Crocodiles}} \\ 
        \hline
        \text{DeepWalk} &H      &$\underset{ .001}{\ufirst{.981}}$&$\underset{ .001}{.799}$
        % &$\underset{ .002}{.781}$
        &$\underset{ .003}{.750}$
        % &$\underset{ .002}{.974}$
        &$\underset{ .001}{.966}$       \\[.92em]
        \text{Node2Vec} &H      &$\underset{ .001}{\ufirst{.982}}$&$\underset{ .001}{.822}$
        % &$\underset{ .005}{.810}$
        &$\underset{ .003}{.780}$
        % &$\underset{ .001}{\ufirst{.979}}$
        &$\underset{ .001}{.973}$       \\[.92em]
        \text{LINE}$_2$ &$l_1$  &$\underset{ .001}{.924}$&$\underset{ .002}{.913}$
        % &$\underset{ .002}{.882}$
        &$\underset{ .001}{.855}$
        % &$\underset{ .003}{.922}$
        &$\underset{ .001}{.930}$       \\[.92em]
        \text{Walklets} &$l_1$  &$\underset{ .001}{\ufirst{.980}}$&$\underset{ .001}{.932}$
        % &$\underset{.002}{\ufirst{.898}}$
        &$\underset{ .001}{.870}$
        % &$\underset{ .004}{.961}$
        &$\underset{ .001}{\ufirst{.976}}$  \\
        \hline
        \text{TADW}     &H      &$\underset{ .001}{.973}$&$\underset{ .001}{.915}$
        % &$\underset{ .003}{.886}$
        &$\underset{ .001}{\ufirst{.884}}$
        % &$\underset{ .002}{.964}$
        &$\underset{ .001}{.967}$       \\[.92em]
        \text{AANE}     &H      &$\underset{ .002}{.911}$&$\underset{ .002}{.772}$
        % &$\underset{ .003}{.833}$
        &$\underset{ .002}{.811}$
        % &$\underset{ .005}{.917}$
        &$\underset{ .005}{.892}$       \\[.92em]
        \text{ASNE}     &H      &$\underset{ .001}{.973}$&$\underset{ .001}{.912}$
        % &$\underset{ .003}{.883}$
        &$\underset{ .002}{.866}$
        % &$\underset{ .005}{.945}$
        &$\underset{ .001}{.940}$       \\[.92em]
        \text{BANE}     &H      &$\underset{ .002}{.653}$&$\underset{ .003}{.664}$
        % &$\underset{ .009}{.659}$
        &$\underset{ .002}{.816}$
        % &$\underset{ .014}{.578}$
        &$\underset{ .002}{.738}$       \\[.92em]
        \text{TENE}     &$l_1$  &$\underset{ .001}{.940}$&$\underset{ .001}{\ufirst{.942}}$
        % &$\underset{ .004}{.857}$
        &$\underset{ .001}{.837}$
        % &$\underset{ .003}{.945}$
        &$\underset{ .001}{.927}$       \\[.92em]
        \hline 
        \textit{AE}     &$l_1$  &$\underset{ .001}{.968}$&$\underset{ .001}{.889}$
        % &$\underset{ .001}{.871}$
        &$\underset{ .002}{.870}$
        % &$\underset{ .002}{.955}$
        &$\underset{ .002}{.952}$       \\[.92em]
        \textit{AE-EGO} &$l_1$  &$\underset{ .001}{.973}$&$\underset{ .001}{.891}$
        % &$\underset{ .002}{.872}$
        &$\underset{ .002}{.872}$
        % &$\underset{ .002}{.953}$
        &$\underset{ .001}{.955}$       \\[.92em]
        \textit{MUSAE}  &$l_1$  &$\underset{ .001}{.973}$&$\underset{ .001}{.908}$
        % &$\underset{ .002}{.885}$
        &$\underset{ .002}{.879}$
        % &$\underset{ .003}{.956}$
        &$\underset{ .001}{.967}$       \\[.92em] 
        \textit{MUSAE-EGO}&$l_1$&$\underset{ .001}{.977}$&$\underset{ .001}{.911}$
        % &$\underset{ .002}{.891}$
        &$\underset{ .002}{\ufirst{.884}}$
        % &$\underset{ .003}{.955}$
        &$\underset{ .001}{.963}$       \\[.92em]
        \hline 
    \end{tabular}
    }

\end{table}






% \begin{table}[htbp!]
%     % \vspace{10pt}
%     \centering
%     \footnotesize
%     \caption{Link prediction performance: average AUC and standard error over 100 seeded runs (best results in red).}
%     \label{tab:link_prediction_1}
%     \resizebox{.49\textwidth}{!}{
%         \vspace{2mm}
%         \begin{tabular}{lcccc}
%             \textbf{}    & \textbf{Facebook} & \textbf{GitHub}& \specialcell{\textbf{Twitch}\\ \textbf{ES}} & \specialcell{\textbf{Wiki}\\\textbf{Crocodiles}} 
%             \\
%             \hline
%             DeepWalk&   {\color{red}$\underset{ .001}{.981}$}      &  $\underset{ .001}{.799}$   &    $\underset{ .002}{.781}$       &  $\underset{ .001}{.966}$    \\[.92em]
%              LINE$_2$ &$\underset{ .001}{.979}$         &  $\underset{ .001}{.899}$   & $\underset{ .003}{.843}$          &   $\underset{ .001}{.938}$   \\[.92em]
%             Node2Vec &   {\color{red}$\underset{ .001}{.982}$ }      &$\underset{ .001}{.822}$     &   $\underset{ .005}{.810}$        &     $\underset{ .001}{.973}$   \\[.92em]
%             Walklets &  {\color{red}$\underset{ \textbf{.001}}{\textbf{.984}}$  }      & $ {\color{red}\underset{ \textbf{.001}}{\textbf{.925}}}$    &    $\underset{ .003}{.873}$   &    {\color{red} $\underset{ \textbf{.001}}{\textbf{.980}}$}\\ \hline
%             TADW &$\underset{ .001}{.973}$&$\underset{ .001}{.915}$&{\color{red}$\underset{ \textbf{.003}}{\textbf{.886}}$}&$\underset{ .001}{.967}$
%                  \\[.92em]
%             AANE & $\underset{ .002}{.911}$&$\underset{ .002}{.772}$&$\underset{ .003}{.833}$&$\underset{ .005}{.892}$ \\[.92em]
%             ASNE &$\underset{ .001}{.973}$&$\underset{ .001}{.912}$&{\color{red}$\underset{ .003}{.883}$}&$\underset{ .001}{.940}$\\[.92em]
%             BANE &$\underset{ .002}{.653}$&$\underset{ .003}{.664}$&$\underset{ .009}{.659}$&$\underset{ .002}{.738}$\\[.92em]
%             TENE &$\underset{ .012}{.735}$&$\underset{ .009}{.878}$&$\underset{ .007}{.722}$&$\underset{ .015}{.872}$\\[.92em]
%             \hline
%             \textit{AE}&$\underset{ .001}{.926}$&$\underset{ .002}{.814}$&$\underset{ .003}{.743}$&$\underset{ .001}{.949}$   \\[.92em]                                                 
%             \textit{MUSAE}& $\underset{ .001}{.945}$&$\underset{ .002}{.917}$&$\underset{ .005}{.871}$&$\underset{ .001}{.968}$    \\ [.92em] 
%             \textit{AE-EGO}&$\underset{ .001}{.928}$&$\underset{ .002}{.786}$&$\underset{ .006}{.727}$&$\underset{ .001}{.939}$   \\[.92em]                                                 
%             \textit{MUSAE-EGO}& $\underset{ .001}{.938}$&$\underset{ .002}{.911}$&{\color{red}$\underset{ .003}{.881}$}&$\underset{ .001}{.969}$     \\ [.92em]              
%              \hline
%         \end{tabular}
%     }
%     \vspace{-5mm}
% \end{table}

